A highly efficient asymptotic preserving IMEX method for the quantum BGK equation

This paper presents an asymptotic preserving (AP) implicit-explicit (IMEX) scheme for solving the quantum BGK equation using the Hermite spectral method. The distribution function is expanded in a series of Hermite polynomials, with the Gaussian function serving as the weight function. The main challenge in this numerical scheme lies in efficiently expanding the quantum Maxwellian with the Hermite basis functions. To overcome this, we simplify the problem to the calculation of polylogarithms and propose an efficient algorithm to handle it, utilizing the Gauss-Hermite quadrature. Several numerical simulations, including a spatially 2D lid-driven cavity flow, demonstrate the AP property and remarkable efficiency of this method.

==> article_integral.tex <==
\section{Multi-dimensional Fermi-Dirac and Bose-Einstein integrals}
\label{sec:integral}
In this section, a numerical evaluation is presented for the Fermi-Dirac and Bose-Einstein integrals \eqref{eq:def_integral}. Then we compare this algorithm to the function \textbf{polylog} to show its efficiency and accuracy.   

\subsection{Numerical algorithm}
We first introduce the algorithm of the integrals in \eqref{eq:def_integral}.  
Enlightened by the derivation of \eqref{eq:int2poly}, we find a relationship between the polylogarithm and the one-dimensional Fermi-Dirac (or Bose-Einstein) integral, which reads
\begin{equation}
    \label{eq:rela-Li}
    \begin{split}
        \int_{\bbR}\frac{1}{\exp\left({\frac{x^2}{2}}\right)-y}|x|^n \rd x&=\frac1y\int_{\bbR}\sum_{k=1}^{\infty}\left(y\exp\left(-\frac{x^2}{2}\right)\right)^k|x|^n\rd x \\
        &=\frac{1}{y}\sum_{k=1}^{\infty}y^kk^{-\frac{n+1}2}2^{\frac{n+1}2}\Gamma\left(\frac{n+1}2\right)\\
        &=\Gamma\left(\frac{n+1}2\right)2^{\frac{n+1}2}\frac{1}{y}\Li_{\frac{n+1}2}(y),
    \end{split}
\end{equation}
then the polylogarithm can be computed with
\begin{equation}
    \label{eq:algo-Li}
    \Li_{s}(y)=y\frac{2^{-s}}{\Gamma\left(s\right)}\int_{\bbR}\frac{1}{\exp\left({\frac{x^2}{2}}\right)-y}|x|^{2s-1} \rd x,
\end{equation}
The right-hand side in \eqref{eq:algo-Li} is the Fermi-Dirac (or Bose-Einstein) integral of only one dimension, which can be approximated by numerical quadrature with tolerable computational cost. 

As shown in Sec. \ref{sec:application}, in the realistic quantum kinetic theory of $d=3$, we always need to calculate the integrals in \eqref{eq:def_integral} with even integers $\alpha_i$. It can be observed from \eqref{eq:int2poly} that we need to compute the polylogarithms with a half-integer $s\geqslant1.5$ (i.e. $2s$ is an integer but $s$ isn't) most frequently. Thus, we will focus on how to compute these polylogarithms with \eqref{eq:algo-Li}.
\begin{remark}
    For general $s$, our method will also give a good approximation of $\Li_s(y)$. Besides, one can transform the integral \eqref{eq:algo-Li} into the form $\int_0^{\infty}\frac{x^n}{\exp(x)-y}\rd x,$ %(i.e. let $x\to\sqrt{2x}$)
    and adopt another method to obtain a better result. We refer the readers to \cite{Gautschi1992} for some possible schemes.
\end{remark}

% Assume that $T$ and $z$ are known, and we will provide the algorithm of $Q_{\alpha}$ in this section.
% Without loss of generality, we suppose $\bu=0$ with a proper frame of reference. 

% To obtain $Q_{\alpha}$ in \eqref{eq:Qalpha}, we only need to compute the moments $\int_{\bbR^3}\mM_q(\bv)\bv^{\alpha}\rd\bv$ and utilize the exact expansion of Hermite polynomials \eqref{eq:form_Hermite}, where $\alpha=(\alpha_1,\alpha_2,\alpha_3)\in\bbN^3$ and $\bv^{\alpha}=v_1^{\alpha_1}v_2^{\alpha_2}v_3^{\alpha_3}$. Obviously, $\int_{\bbR^3}\mM_q(\bv)\bv^{\alpha}\rd\bv=0$ if $\alpha$ contains any odd index. 

% On the other hand, when all indices of $\alpha$ are even and $|z\theta_0|<1$, it holds 
% \begin{equation}
%     \label{eq:mom_M}
%     \begin{split}
%         \int_{\bbR^3}\mM_q(\bv)\bv^{\alpha}\rd \bv&=\int_{\bbR^3}\frac{1}{z^{-1}
%         \exp\left(\frac{\bv^2}{2T}\right)+\theta_0}\bv^{\alpha}\rd \bv \\
%         &=\int_{\bbR^3}z\exp\left(-\frac{\bv^2}{2T}\right)\frac{1}{1+z\theta_0\exp\left(-\frac{\bv^2}{2T}\right)} \bv^{\alpha}\rd \bv \\
%         &=-\frac{1}{\theta_0}\int_{\bbR^3}\sum_{n=1}^{\infty}\left[-z\theta_0\exp\left(-\frac{\bv^2}{2T}\right)\right]^n\bv^{\alpha}\rd\bv \\
%         &=-\frac{(\alpha-1)!!}{\theta_0}\sum_{n=1}^{\infty}(-z\theta_0)^n\left(\frac{T}{n}\right)^{\frac{|\alpha|+3}2} \\
%         &=-\frac{(\alpha-1)!!}{\theta_0}(2\pi)^{\frac32}T^{\frac{|\alpha|+3}2} \Li_{\frac{|\alpha|+3}2}(-z\theta_0),
%     \end{split}
% \end{equation}
% where $(\alpha-1)!!=(\alpha_1-1)!!(\alpha_2-1)!!(\alpha_3-1)!!$ and $(-1)!!$ is regarded as $1$. Besides, 
%  In fact, for both the integral in \eqref{eq:mom_M} and the polylogarithm ($s>1$), the analytic continuation w.r.t. $-z\theta_0$ and $y$ is available on $(-\infty, 1]$. Thus, \eqref{eq:mom_M} holds for any $z\theta_0\ge-1$. 

% Since the exact form of Hermite polynomials can be written out, we only need to approximate \eqref{eq:mom_M} to obtain $Q_{\alpha}$. One way is to numerically calculate the integration on the left-hand side, which will consume large computational costs due to the high dimensionality. 
% Another way is to approximate the polylogarithm on the right-hand side. 


% In fact, a method to compute $\Li_s(y)$ for $s>1$ and $y\leqslant1$ can meet our demands.  
% and 

The Gauss-Hermite quadrature is often adopted to deal with the integral on $(-\infty, \infty)$, which has the form
\begin{equation}
    \label{eq:GH-quad}
    \int_{\bbR}g(x)\exp(-x^2)\rd x\approx \sum_{k=1}^N \omega_kg(x_k),
\end{equation}
where $x_k$ are the roots of $(N+1)-$degree Hermite polynomial, and $\omega_k$ are the weights. The detailed calculations of $x_k$ and $\omega_k$ will not be discussed here, and a feasible approach can be referred to \cite{Glaser2007}. It is always difficult to accurately calculate $x_k$ and $\omega_k$ when $N$ is too large, so we take $N=70$ in all the following tests. 

In practice, the Gauss-Hermite quadrature is always utilized in the rescaled form 
\begin{equation}
    \label{eq:rescale-GH}
    \int_{\bbR}g(x)\exp\left(-\frac{x^2}{\beta}\right)\rd x=\sqrt{\beta}\int_{\bbR}g(\sqrt{\beta}x)\exp\left(-{x^2}\right)\rd x\approx \sqrt{\beta}\sum_{k=1}^N \omega_kf(\sqrt{\beta}x_k),
\end{equation}
where $\beta$ is some positive constant. Then the integral in \eqref{eq:algo-Li} can be approximated with
\begin{equation}
    \label{eq:GH-Li}
    \int_{\bbR}\frac{1}{\exp\left({\frac{x^2}{2}}\right)-y}|x|^{2s-1}\rd x=\int_{\bbR}\exp\left(-\frac{x^2}{\beta(s,y)}\right)G(x,y)\rd x=\sqrt{\beta(s,y)}\sum_{k=1}^N \omega_k G(\sqrt{\beta(s,y)}x_k,y),
\end{equation}
where 
\begin{equation}
    \label{eq:def-G}
    G(x,y)=\frac{\exp\left(\frac{x^2}{\beta(s,y)}\right)}{\exp\left({\frac{x^2}{2}}\right)-y}|x|^{2s-1}.
\end{equation}
and $\beta(s,y)$ is a positive function to be determined. 
%From the convergence theory of Gauss-type quadrature, when $G(\cdot,y)$ behaves close to a polynomial, the approximation will be more accurate. 

\paragraph{Fitting $\beta(s,y)$}
With some fundamental observations, we find that when $y$ is close to $1$, the integral becomes more singular at $x=0$. Therefore, the integral near $y=1$ is more difficult to calculate and requires a careful choice of $\beta$. On the other hand, in the area far from $y=1$, we may obtain an excellent approximation with a wide range of $\beta$. Besides, when $s$ gets larger, the singularity will become weaker and we can get a good approximation more easily.

Hence, we focus on how to choose $\beta$ for $s=1.5, 2.5$ and $y$ is close to $1$. Without any prior knowledge, the optimal $\beta$ is calculated for $y\in[0.9,1]$ with interval $0.001$. It is observed that the results of $\beta$ are well fit with a linear function of $y$, which are displayed in Fig. \ref{fig:opt_beta}.
\begin{remark}
    There exists a gap of optimal $\beta$ owing to $\Li_s(y)$ is not analytic near $y=1$. The result at $y=1$ is excluded from our fitting data.
\end{remark}

\begin{figure}[!htb]
  % \colorbox{black}
    \centering
      \subfloat[Optimal $\beta$ in \eqref{eq:GH-Li} of $s=1.5$.]
    {\includegraphics[width=0.45\textwidth, height=0.36\textwidth,
      clip]{image/fitting/s=1.5.png}}\hfill
      \subfloat[Optimal $\beta$ in \eqref{eq:GH-Li} of $s=2.5$.]
    {\includegraphics[width=0.45\textwidth, height=0.36\textwidth,
      clip]{image/fitting/s=2.5.png}}\hfill
      \caption{The results of $\beta$ in the numerical quadrature \eqref{eq:GH-Li} for $s=1.5$ and $s=2.5$. Blue lines are the optimal $\beta$. Red lines correspond to the fitting results $\beta=1.914-1.767y$ for $s=1.5$, and $\beta=1.483-1.224y$ for $s=2.5$.}
    \label{fig:opt_beta}
\end{figure}
Besides, we find that $\beta=1$ can lead to an accurate approximation when $y<0$. 
With these attempts and explorations, we decide to take $\beta(s,y)$ as
\begin{equation}
    \label{eq:beta_y}
    \beta(s,y)=\left\{\begin{array}{ll}
        A(s)-B(s)y, & 0\leqslant y\leqslant 1, \\
        1, &  y<0,
    \end{array}
    \right.
\end{equation}
where $A(s)=1+2.379\exp(-0.638s),\; B(s)=0.5-0.626\exp(-0.382s)-A(s)$, which is obtained based on the results of $s=1.5$ and $s=2.5$.

For now, we have formulated an algorithm of $\Li_s(y)$ for $s>1, y\leqslant 1$, which can be summarized as Algorithm \ref{algo:polylog}. 
\begin{algorithm}[htbp]
    \caption{Numerical algorithm of $\mI(\alpha, C, y)$ in \eqref{eq:def_integral}}
    \label{algo:polylog}
    \begin{algorithmic}[1]
        \item Decide the parameter $\beta\left(\frac{|\alpha|+d}{2}, y\right)$ with \eqref{eq:beta_y}.
        \item Compute the polylogarithm $\Li_{\frac{|\alpha|+d}{2}}(y)$ with \eqref{eq:algo-Li} and \eqref{eq:GH-Li}.
        \item Compute $\mI(\alpha, C, y)$ with \eqref{eq:int2poly}.
    \end{algorithmic}
\end{algorithm}

\subsection{Comparison to \textbf{polylog} in MATLAB} 
To validate this method, we record the error $e=\Li_{\rm num}-\Li_{\rm ref}$ for $s=1.5, 2.5, 3.5$ and $y\in[-10,1]$ with interval $0.01$. Here $\Li_{\rm num} $ corresponds to the result of our method, and $\Li_{\rm ref}$ is the reference result by MATLAB's function \textbf{polylog}. 

\begin{figure}[!htb]
  % \colorbox{black}
    \centering
      \subfloat[Error of $\Li_{1.5}(y)$.]
    {\includegraphics[width=0.3\textwidth, height=0.24\textwidth,
      clip]{image/error_polylog/s=1.5.png}}\hfill
      \subfloat[Error of $\Li_{2.5}(y)$.]
    {\includegraphics[width=0.3\textwidth, height=0.24\textwidth,
      clip]{image/error_polylog/s=2.5.png}}\hfill
      \subfloat[Error of $\Li_{3.5}(y)$.]
    {\includegraphics[width=0.3\textwidth, height=0.24\textwidth,
      clip]{image/error_polylog/s=3.5.png}}\hfill
      \caption{The error of $\Li_s(y), \; s=1.5,2.5,3.5$ with Algorithm \ref{algo:polylog}. MATLAB's function \textbf{polylog} is taken to compute the reference results.} 
    \label{fig:polylog}
\end{figure}
It can be observed in Fig. \ref{fig:polylog} that we can obtain reliable results with Algorithm \ref{algo:polylog}. To further show the efficiency of our scheme, we record the running time of both methods, which are given in Tab. \ref{table:polylog_time}.

\begin{table}[!ht]
\centering
\def\arraystretch{1.5}
{\footnotesize
\begin{tabular}{llll}
\hline
    & s=1.5 & s=2.5 & s=3.5        \\
\hline
Our method & $4.2\times10^{-3}$s & $1.23\times10^{-2}$s & $1.16\times10^{-2}$s\\
\textbf{polylog} & 39.52s & 38.35s & 44.14s\\
\hline
\end{tabular}
}
\caption{Total running time (on MATLAB R2020b) in the experiment of polylogarithm in Sec. \ref{sec:integral}.}
\label{table:polylog_time}
\end{table}

\begin{remark}
    As observed in Fig. \ref{fig:polylog}, the results on $[-10, 0.9]$ are more accurate than on $[-10, 1]$. Thus, one may adopt this method on $y\leqslant0.9$ and call the function \textbf{polylog} on $[0.9,1]$, which will achieve higher accuracy and also save many computational assumptions than directly using \textbf{polylog}.

    In our numerical experiments of the quantum BGK model, all results are obtained with Algorithm \ref{algo:polylog}.
\end{remark}

As can be observed in Tab. \ref{table:polylog_time}, our method is thousands of times faster than the function \textbf{polylog} in MATLAB! Under the c++ environment, our algorithm will get even faster. 

Up to now, we have completed a highly efficient scheme of the Fermi-Dirac (or Bose-Einstein) type integrals \eqref{eq:def_integral}. In the next section, we will apply this method to the numerical simulations of quantum kinetic problems.  


